Informed Proposal Monte Carlo

Any search or sampling algorithm for solution of inverse problems needs guidance to be efficient. Many algorithms collect and apply information about the problem on the fly, and much improvement has been made in this way. However, as a consequence of the the No-Free-Lunch Theorem, the only way we can ensure a significantly better performance of search and sampling algorithms is to build in as much information about the problem as possible. In the special case of Markov Chain Monte Carlo sampling (MCMC) we review how this is done through the choice of proposal distribution, and we show how this way of adding more information about the problem can be made particularly efficient when based on an approximate physics model of the problem. A highly nonlinear inverse scattering problem with a high-dimensional model space serves as an illustration of the gain of efficiency through this approach.

==> 1-MC Inversion Guided by Simplified Physics - Basic Theory/MC-with-Phys-Proposals-170919.tex <==
\input{preample.tex}

\begin{document} 
\title{\bf Monte Carlo Sampling with\\ Problem-dependent Proposals}
%\date{ } 

%\thispagestyle{empty}
%\vspace*{10mm}
%\bigskip
\author{Klaus Mosegaard${}^{1}$ \\ Sarouyeh Khoshkholgh${}^{1}$ \\ Others ?$\dots$}
\date{}
\maketitle

{\begin{center}
{${}^1$ Department of Physics of Ice, Climate and Earth, Tagensvej 16, 2200 Copenhagen N, Denmark}
\end{center}
%\vspace*{2mm}
%\begin{center}
%{${}^2$Department of Earth Sciences \\ ETH Zuerich,
%Sonneggstrasse 5, 8092 Zuerich Switzerland} 
%\vspace*{10mm}
%%\\ {Klaus Mosegaard  \\  2004}
%\end{center}
}

\setcounter{page}{0}

%
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
%\clearpage
%
%\tableofcontents
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
%\clearpage

\begin{abstract}
Abstract abstract abstract abstract abstract abstract abstract abstract 
\end{abstract}

\section{Introduction}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
Introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction  
 
\section{Classical MCMC}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
In this section we follow Tarantola and Valette (1982a) whose formulation of the probabilistic inference problem is based on an expression for the conjunction of information given by two probability densities $f_1(\bfx)$ and $f_2(\bfx)$ over the same space $\calX$:
$$
(f_1 \wedge f_2) (\bfx) = \frac{f_1(\bfx) f_2(\bfx)}{\mu(\bfx)}.
$$ 
where ${\mu(\bfx)}$ is the homogeneous probability density assigning equal probabilities to equal volumes in $\calX$.
They adapt this formula to the inference problem by defining $\bfx = (\bfd,\bfm)$ as a point in the joint data-model space, and obtain the posterior probability distribution:
$$
\sigma(\bfd,\bfm) = \frac{\rho(\bfd,\bfm) \theta(\bfd,\bfm)}{\mu(\bfd,\bfm)}.
$$
Under the assumption that the priors over $\bfd$ and $\bfm$ are independent, that is, $\rho(\bfd,\bfm)=\rho_d(\bfd) \rho_m(\bfm)$, that $\mu(\bfd,\bfm)$ is constant, and that the physical relation $\bfd = \bfg(\bfm)$ is exact, such that $\theta(\bfd,\bfm)=\delta(\bfd - \bfg(\bfm)) \mu(\bfm)$, we arrive at an expression for the posterior in the model space
\begin{equation}
\sigma_m(\bfm) = L(\bfm)\rho_m(\bfm)
\label{TV-Bayes}
\end{equation} 
with
$L(\bfm)=\rho_d(\bfg(\bfm)).$
Equation (\ref{TV-Bayes}) is equivalent to the classical Bayes Formula, which in our notation reads
$$
\sigma_m(\bfm | \bfd) = \frac{L(\bfd | \bfm)\rho_m(\bfm)}{\rho_d(\bfd)}.
$$
The posterior distribution (\ref{TV-Bayes}) is generally impossible to calculate directly, except for linear inverse problems, so one has to rely on Monte Carlo sampling methods to generate realizations from the distribution. A commonly used approach is the Extended Metropolis Algorithm (\cite{MT95,M06}):

\bigskip\noindent
\begin{Algorithm}
\label{algo: ext-Metro}
\textbf{(Extended Metropolis).} Given a random algorithm $V\left( \mathbf{m}\right) 
$ which iteratively samples the prior probability density ${\rho_m (\mathbf{m})}$: 
\begin{equation}
\mathbf{m}^{(n+1)}=V\left( \mathbf{m}^{(n)}\right) ,  \label{eq: priorwalk}
\end{equation}
and an algoritm $U\left( 0,1\right) $ producing random numbers from the interval $\left[ 0,1\right]$ with uniform probability. The random algorithm $W$, which iteratively updates the current parameter vector $\mathbf{m}^{(n)}$: 
\begin{equation}
\mathbf{m}^{(n+1)}=W\left( \mathbf{m}^{(n)}\right) =\left\{ 
\begin{array}{l}
V\left( \mathbf{m}^{(n)}\right) \text{ if }U\left( 0,1\right) \leq \min
\left[ 1,\frac{L\left( V\left( \mathbf{m}^{(n)}\right) \right) }{L\left( 
\mathbf{m}^{(n)}\right) }\right]  \\ 
\mathbf{m}^{(n)}\text{ else}
\end{array}
,\right.   \label{bigwalk}
\end{equation}
will asymptotically sample the posterior ${\sigma (\mathbf{m}) \propto L(\mathbf{m})\rho (%
\mathbf{m})}$.
\end{Algorithm}

\bigskip\noindent
Algorithm~\ref{algo: ext-Metro} works if the prior sampler $V$ is {\em irreducible} and {\em aperiodic} (see, e.g., \cite{MT02}). 

\bigskip\noindent
The extended Metropolis will, in general, perform better than a regular Metropolis, since only models that are accepted a priori (by $V$) will be subject to the time consuming misfit calculation needed to evaluate $L({\bf m}) $.

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
\section{No-Free-Lunch Theorems and the importance of information}
\label{sec:NFL}
Text text text text text text text text text text text text text  


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
\section{Blind and Informed Proposals Mechanisms}
Despite the improved efficiency of Algorithm (\ref{algo: ext-Metro}) gained from the use of a prior sampler $V$ in the initial phase of each algorithm, practical experience shows that the efficiency of extended Metropolis is highly dependent on the choice of $V$. The problem is that the prior $\rho$ and the likelihood function $L$ are usually so different that the moves in the model space proposed by $V$ will usually lead to points with low values of $L$. As explained earlier, there is little hope that even the best, blind sampling strategy will be able to significantly improve on this problem. In the following we shall therefore describe a method that will allow us to inject information about the physical relation between data and model parameters into the sampling strategy. First, however, we will understand why the 'blind' strategy of the classical MCMC is so inefficient.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Proposal Distributions in Classical MCMC}
The basic idea behind any implementation of the Metropolis Algorithm is an interplay between {\em proposals} and {\em rejections}. In each iteration, sampling from a probability density $f(\bfx)$ over a space $\calX$ proceeds from a current value $\bfx$ by first proposing a new value ${\bfx}'$ from the so-called {\em proposal distribution} $q({\bfx}',\bfx)$, followed by a random decision where ${\bfx}'$ is accepted with probability
%
\begin{equation}
P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}={\rm min} \( \frac{f({\bfx}') q(\bfx|{\bfx}')}{f(\bfx) q({\bfx}'|\bfx)},1 \).
\end{equation}
%
This follows from the requirement that the probability that a transition takes place from $\bfx$ to ${\bfx}'$, namely
$P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'} q({\bfx}'|\bfx) f(\bfx)$, must be equal to the probability of the reverse transition
$P_{\rm acc}^{{\bfx}' \rightarrow {\bfx}} q(\bfx|{\bfx}') f({\bfx}')$ to attain equilibrium sampling (detailed balance). At this point it is important to note that the proposal distribution has no influence on the distribution to which the sampling converges, it only influences the speed of convergence. 

It is common practice (but not a necessity) to work with symmetric proposal distributions: $q({\bfx}',\bfx) = q(\bfx , {\bfx})$, and in this case we get the simpler expression
\begin{equation}
P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}={\rm min} \( \frac{f({\bfx}')}{f(\bfx)},1 \).
\label{eq_accept}
\end{equation}
%
The Metropolis sampler is only efficient if large enough steps (to connect any two high value areas of $f(\bfx)$ in a few steps) will be frequently accepted. This ability critically depends on the $q({\bfx}',\bfx)$, and that is reason why intensive research in recent years has been devoted to finding improved proposal distributions. 

A close look at the expression for the unconditional transition probability from $\bfx$ to $\bfx'$ (for symmetric $q$)
\begin{equation}
P^{{\bfx} \rightarrow {\bfx}'}=f(\bfx) P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}=f(\bfx) \cdot q({\bfx}'|\bfx) \cdot {\rm min} \( \frac{f({\bfx}')}{f(\bfx)},1 \).
\end{equation}
shows that, if $f(\bfx)'$ turns out to be low  in places where $q({\bfx}'|\bfx)$ is high, the move ${\bfx} \rightarrow {\bfx}'$ is very likely to be rejected. 

To investigate and exemplify the importance of this problem in high-dimension\-al spaces, let us consider the case where the distribution of ${\bfx}$ is Gaussian with covariance matrix $\bfC$ and mean $\bfx_0$:
$f({\bfx}) = \calN_{\bfx} (\bfx_0,\bfC)$.
Assume now that out proposal distribution is an isotropic Gaussian $q({\bfx}|{\bfx}_q) = \calN_{\bfx} (\bfx_q,\bfC_q)$ with mean ${\bfx}_q$ and covariance matrix $\bfC_q$, 
and that we, in the sampling process, have arrived at point with a high value of $f({\bfx})$, say, for simplicity, at its maximum point ${\bfx}_0$. We can now calculate the expected acceptance probability $P^{{\bfx}_0 \rightarrow {\bfx}}$ proposed in the next step by the algorithm:
\begin{align}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) 
&= \int_{\calX} \frac{f({\bfx})}{f({\bfx}_0)} q({\bfx}|{\bfx}_0) d{\bfx} \label{eq: Meanf1} \\
&= \int_{\calX} \frac{\calN_{\bfx} (\bfx_0,\bfC)}{\calN_{\bfx_0} (\bfx_0,\bfC)} \calN_{\bfx} (\bfx_0,\bfC_q) d{\bfx} \\
&= \frac{\calN_{\bfx_0} (\bfx_0,\bfC+\bfC_q)}{\calN_{\bfx_0} (\bfx_0,\bfC)}\int_{\calX} 
\calN_{\bfx} (\bfx_1,\bfC_1) d{\bfx} 
\label{eq: Meanf}
\end{align}
where
\begin{equation*}
\bfx_1 
= (\bfC^{-1} + \bfC_q^{-1})^{-1} (\bfC^{-1} \bfx_0 + \bfC_q^{-1} \bfx_0) = \bfx_0
\end{equation*}
and 
\begin{equation*}
\bfC_1 = (\bfC^{-1} + \bfC_q^{-1})^{-1} \, .
\end{equation*}
Since the integral in (\ref{eq: Meanf}) is $1$, we have the following expression for the expected acceptance probability:
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) = \frac{\calN_{\bfx_0} (\bfx_0,\bfC+\bfC_q)}{\calN_{\bfx_0} (\bfx_0,\bfC)} 
= \( \frac{{\rm det}\( 2\pi \bfC \)}{{\rm det}\( 2\pi (\bfC+\bfC_q) \)} \)^{1/2} \, .
\end{equation}
Both $\bfC_q = \sigma_q^2 {\bfI}$ (with $\sigma_q^2 > 0$) and $\bfC$ are diagonal in the frame spanned by $\bfC$'s eigenvectors, and if we assume that the eigenvalues of $\bfC$ are $\sigma_1^2 \ge \dots \ge \sigma_N^2 > 0$, where $N$ is the dimension of $\calX$, the eigenvalues of $\bfC+\bfC_q$ are
$(\sigma_1^2+\sigma_q^2), \dots ,(\sigma_N^2+\sigma_q^2)$. From this we have  
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) = \prod_{n=1}^N
\( \frac{\sigma_n^2}{\sigma_n^2+\sigma_q^2}
\)^{1/2} \, .
\label{eq-eigenC1}
\end{equation}
From (\ref{eq-eigenC1}) we see that for any non-zero values of $\sigma_n$ and $\sigma_q$ we have 
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) \rightarrow 0 \quad {\rm for} \quad N \rightarrow  \infty \, .
\end{equation}
expressing the influence on sampling of the so-called 'curse of dimensionality'. If the proposed steps are kept very short ($\sigma_q$ is small compared to all $\sigma_n$), the decrease of $E(P^{{\bfx}_0 \rightarrow {\bfx}})$ with $N$ is slow. But this situation is of no practical value, because adequate sampling by the algorithm requires that it can traverse high-probability areas of $f({\bfx})$ within a reasonable amount of time. 

For non-negligible step lengths, the situation is radically different. Indeed, if there exists an integer $K$ and a real constant $k$ such that $\sigma_q > k\sigma_n$ for all $n > K$, then $E(P^{{\bfx}_0 \rightarrow {\bfx}})$ decreases more that exponentially with $N$. In other words, if the distribution $f({\bfx})$ is 'elongated' compared to the proposal $q$, that is, if it is broader than $q$ in only a finite number of directions/dimensions, the mean number of accepted moves will decrease at least exponentially with the number of dimensions.

As an example, let us consider the case where $\sigma_q^2 = 1$, and $\sigma_n^2 = 1/n$. For $N=2$ this gives an expected acceptance probability of $0.4082$, corresponding to a mean waiting time of about $0.4082^{-1} \approx 2.5$ iterations between accepted moves. For $N=10$ the expectation is $1.5828 \cdot 10^{-4}$, and for $N=100$ it decreases to $1.03 \cdot 10^{-80}$, giving a waiting time of about $3.0 \cdot 10^{62}$ years for 1 Billion iterations per second.

The above analysis is carried out under the very favourable situation where the maximum of $f({\bfx})$ has been located by the algorithm, and does not even consider the serious difficulties faced by the sampling algorithm in the initial search for points with high values of $f({\bfx})$ (the {\em burn in} phase). So it is clear that the proposal mechanism, as defined by $q$, is the Achilles heel of the standard MCMC approach.
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Sampling with Problem-dependent Proposals}
The unsurmountable difficulties described in the previous section are rooted in the fact that standard MCMC calculations are essentially blind search algorithms supplemented with a few problem-specific features. To evade the fundamental problems of classical MCMC sampling, we shall therefore take the consequence of the legacy of the No-Free-Lunch theorem and propose a class of algorithms that explicitly incorporates information about the problem to be solved.

To avoid a mismatch between the distribution $f({\bfx})$ to be sampled, and the proposal distribution $q(\bfx' | \bfx)$, we shall in the following look into proposals $q$ that are approximations to $f$, in the sense that 
\begin{equation}
q(\bfx' | \bfx) = \tilde{f} ({\bfx'})
\end{equation}
where the Kullbach-Leibler divergence
\begin{equation}
D(f,\tilde{f}) = \int_\calX f({\bfx}) \log \( \frac{f({\bfx})}{\tilde{f}(\bfx)} \) d{\bfx}
\end{equation}
is small. For a given inverse problem, the challenge is here to derive $\tilde{f}({\bfx})$. We shall devote the next section to this problem, where the focus will be on the special conditions characterizing inverse problems. 

\subsection{Inverse Problems: proposing through approximate forwards} 
When applying an MCMC method to inverse problems, where $f(\bfx)$ is the posterior $\sigma(\bfx)$ or the likelihood $L(\bfx)$, the expected acceptance probability is given by (\ref{eq: Meanf1}). This expression is largest (equal to $1$) when $f({\bfx}_0) = q({\bfx}|{\bfx}_0)$ for all $\bfx$, or, when $q$ is symmetric, $f({\bfx}) = q({\bfx}|{\bfx}_0)$ for all $\bfx_0$. In case $q({\bfx}|{\bfx}_0)$ deviates from $f(\bfx)$ there will be areas within $\calX$ where $q({\bfx}|{\bfx}_0)<f(\bfx)$ as well as areas with  $q({\bfx}|{\bfx}_0)>f(\bfx)$, because both $f$ and $q({\bfx}|{\bfx}_0)$ are positive with integral $1$ over $\calX$. It is, however, the areas with $q({\bfx}|{\bfx}_0)<f(\bfx)$ that are critical, because they directly reduce the acceptance probability. In the following we exploit this fact to construct approximate likelihood functions or posterior distributions, allowing efficient sampling of solutions to inverse problems.

\subsubsection{Approximate posteriors}
Consider an inverse problem with observational data $\bfd^{obs}$ and computed data 
\begin{equation*}
{\bfd} = {\bfg}({\bfm}) \, .
\end{equation*}
Here, ${\bfg}$ is an exact forward function. Suppose that we also have an approximate forward relation $\tilde{\bfg}$ that allows us efficiently compute approximate data
\begin{equation*}
\tilde{\bfd} = \tilde{\bfg}({\bfm}) \, .
\end{equation*}
and that a (possibly simplified) prior probability density 
$\tilde{\rho}_m({\bfm})$ is available.  With this method in hand we can form an approximate posterior probability distribution
\begin{equation}
\tilde{\sigma}({\bfm}) = \tilde{L}({\bfm}) \tilde{\rho}_m({\bfm}) = \rho_d (\tilde{\bfg}({\bfm})) \tilde{\rho}_m({\bfm})
\end{equation}
which can be used directly as a proposal distribution: 
\begin{equation}
q({\bfm}'|{\bfm}) = \tilde{\sigma}({\bfm}') \, .
\end{equation}
Another approach is to use some 'pseudo-inverse' function 
$\bfh$ (if available) on the observed data $\bfd_{obs}$:
\begin{equation*}
{\bfm}_{est} = {\bfh}(\bfd_{obs}) \, .
\end{equation*}
and to use the image $\sigma_{pseud}$ of the data distribution $\rho_d$ under $\bfh$:
\begin{equation}
\sigma_{pseud}({\bfm})
 = 
\frac{\partial{\tilde{\bfh}}}{\partial{\bfd}}\rho_d({\bfd}) \, .
\end{equation}
as a proposal distribution
\begin{equation}
q({\bfm}'|{\bfm}) = \sigma_{pseud}({\bfm}') \, .
\end{equation}
However, the fact that we can use the above approximations to the posterior as proposals does not mean that they are efficient. In the following sections we shall analyse some necessary conditions for efficiency, and give examples of implementations. The efficiency conditions will, of course, depend on the category of problems we face (linear, mildly non-linear, highly non-linear), so we will consider these situations in turn.

\subsubsection{Linear, Gaussian Problems}
Sampling of solutions to a linear Gaussian problem through rejection sampling is straightforward. We have an explicit expression for the Gaussian posterior, and the distribution itself can be used as an exact proposal. Samples $\bfm$ from an $N$-dimensional standard (isotropic) Gaussian (mean $\bf 0$ and covariance $\bfI$) can be generated with the Box-M\"uller method, and the desired samples ${\bfm}$ from a $N$-dimensional multivariate Gaussian with mean ${\bfm}_0$ and covariance $\bfC$ can be calculated as 
${\bfm} ={\bfm}_0 + {\bfA}{\bfm}$, 
where ${\bfA}{\bfA}^T = {\bfC}$. The matrix ${\bfA}$ can be found by, for instance, Cholesky decomposition.

\subsubsection{Nonlinear Problems}
We shall now propose a procedure for efficient sampling of solutions to nonlinear problems with a homogeneous (constant) prior. 

\medskip
\noindent
Given an inverse problem 
\begin{equation*}
{\bfd} = {\bfg}({\bfm})
\end{equation*}
with homogeneous prior, observed data ${\bfd}_{obs}$, and data covariance matrix $\bfC_d$. The problem is characterized by its likelihood function
$L({\bfm}) = \calN_{\bfd_{obs}}({\bfg}({\bfm}),{\bfC}_d)$. 
and its prior $\rho(\bfm) = \mu(\bfm)$, and will in the following be expressed through the notation
\begin{equation}
\calP = \{ \calN_{\bfd_{obs}}({\bfg}({\bfm}),{\bfC}_d), \mu(\bfm) \} \, .
\end{equation}
We shall furthermore consider an approximation to $\calP$
\begin{equation}
\tilde{\calP} = \{ \calN_{\bfd_{obs}}(\tilde{\bfg}({\bfm}),{\bfC}_d), \mu(\bfm) \} \, ,
\end{equation}
As a measure of the difference between the exact posterior and the approximate posterior in the joint $(\bfd,\bfm)$-space, we shall use the Kullbach-Leibler divergence of the conditional $\sigma(\bfd |\bfm)$:
\begin{align}
D(\sigma(\bfd |\bfm),\tilde{\sigma}(\bfd |\bfm)) 
&= \int_\calX \sigma({\bfd}|{\bfm}) \log \( \frac{\sigma({\bfd}|{\bfm})}{\tilde{\sigma}({\bfd}|\bfm)} \) d{\bfd} \label{eq: Kull} \\
&= \int_\calX \calN_{\bfd}({\bfg}({\bfm}),{\bfC}_d) \log \( \frac{\calN_{\bfd}({\bfg}({\bfm}),{\bfC}_d)}{\calN_{\bfd}(\tilde{\bfg}({\bfm}),{\bfC}_d)} \) d{\bfd} \\
&= \frac{1}{2} \({\bfg}({\bfm})-\tilde{\bfg}({\bfm}))^T {\bfC}_d^{-1} ({\bfg}({\bfm})-\tilde{\bfg}({\bfm})) \) \\
&= \frac{1}{2} \| {\bfg}({\bfm})-\tilde{\bfg}({\bfm}) \|_{{\bfC}_d}^2
\end{align}
which is the ${\calL}_2$-distance with weight matrix ${\bfC}_d$ between the approximate, computed data $\tilde{\bfg}({\bfm})$ and the exact, computed data ${\bfg}({\bfm})$. This shows that the amount of information missing in $\tilde{\calP}$, compared to $\calP$ (the Kullbach-Leibler divergence) can be measured directly from the difference between ${\bfg}({\bfm})$ and $\tilde{\bfg}({\bfm})$.



\medskip\noindent
This suggests the following:
\noindent
\begin{Algorithm}
Use $\calN_{\bfd_{obs}}(\tilde{\bfg}({\bfm}),{\bfC}_d)$ as the proposal distribution in Algoritm (\ref{algo: ext-Metro}).
\label{algo: ext-Metro-KBMC}
\end{Algorithm}

\subsubsection{Example: A 100-parameter inverse scattering problem}
Figure $\dots$ shows acoustic impedances of a 1000-parameter, horizontally stratified earth model, and the vertical-incidence seismic data generated from the model. The data are 1D full-waveform seismic signals, generated and recorded at the surface. The full-waveform data contains all multiple reflections, transmission losses and damping effects, so the inverse problem of recovering the model from the data is highly nonlinear. A linearized approximate solution to the inverse scattering problem (in the absence of noise) is shown to the right. This solution requires very little computation time, but is clearly inaccurate (compare to left graph). A more accurate solution, with uncertainty estimates, can be obtained by Markov chain Monte Carlo (MCMC) if enough samples can be obtained in reasonable time. Figure  $\dots$ (upper curve) shows the lack of convergence to equilibrium of a classical MCMC in the first 2000 iterations of such an inversion process. The lower curve, however, shows much faster convergence of a Algorithm (\ref{algo: ext-Metro-KBMC}) whose random walk is guided by the linearized solution shown in Figure $\dots$. Algorithm (\ref{algo: ext-Metro-KBMC}) uses a forward modeling error distribution centered in the linearized solution to choose samples. The improvement in convergence time is dramatic, in this case of the order of $10^4$ when started at the same model as the Algorithm (\ref{algo: ext-Metro}).


%\begin{figure}[htp]
%
%  \centering
%
%  \label{figur}
%
%  \begin{tabular}{cc}
%
%    % Requires \usepackage{graphicx}
%
%    \framebox{\includegraphics[width=1.8in]{TrueModel-xx.png}}
%    \framebox{\includegraphics[width=1.01in]{dobs.png}}
%    \framebox{\includegraphics[width=1.8in]{ApproxModel.png}} \\
%    
%  \end{tabular}
%  \caption{A 1000-layer, horizontally stratified Earth model (left), the corresponding vertical-incidence, full-waveform seismic data (middle), and a classical, linearized solution to the inverse problem (right).}
%\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{TrueModel-xx.png}
        %\caption{A gull}
        %\label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{dobs.png}
        %\caption{A tiger}
        %\label{fig:tiger}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{ApproxModel.png}
        %\caption{A mouse}
        %\label{fig:mouse}
    \end{subfigure}
    \caption{A 1000-layer, horizontally stratified Earth model (left), the corresponding vertical-incidence, full-waveform seismic data (middle), and a classical, linearized solution to the inverse problem (right).}\label{fig:animals}
\end{figure}



\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{Exp-1-Iter-10000-TrueErrorEnvelope.png}
\caption{Linear Inversion: Modelization Error: True Error Envelope} 
\end{center}
\end{figure}

\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{Exp-1-Iter-10000-EstErrorEnvelope.png}
\caption{Linear Inversion: Modelization Error: Est Error Envelope} 
\end{center}
\end{figure}

\vfill

\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{IMC-MCMC-iter-2000-Misfits-x.png}
\caption{Convergence towards equilibrium of a classical MCMC algorithm (upper curve), attempting to sample solutions to the inverse problem described in Figure 5. Lower curve is the fast-converging KBMC algorithm guided by the linearized inversion. In this case the convergence of the KBMC algorithm was of the order of 104 times faster than the MCMC algorithm.} 
\end{center}
\end{figure}

\vfill

%We will improve algorithm performance by introducing the concept of passive prior information (contrast to usual active prior information used in Bayes Rule). Passive priors carry simplified information about relations between data and unknown model parameters to improve algorithmic convergence, but do not influence the posterior distribution directly. Passive priors can be built from neural networks, simplified physics, or other representations of relations in Nature.



%\vskip 1.5cm
\medskip
\noindent
%
%
%
%\newpage
\subsubsection{Procedure 2: Sampling with General Prior}
({\dots soon to appear\dots)



%\thispagestyle{empty}
%\vspace*{60mm}
\clearpage


%\section{References}

\newcommand{\marginlabel}[1]
   {\mbox{}\marginpar{\raggedleft\hspace{0pt}#1}}

\begin{thebibliography}{999}

%\bibitem{B1773}
%Buffon, G., Memoire sur le jeu de franc-carreau, 1733

%\reversemarginpar

\bibitem{B1777}
Buffon, G., 1777. Essai d'arithmetique morale.

\bibitem{MT95} 
Mosegaard, K., and Tarantola, A., 1995. Monte Carlo sampling of solutions to inverse problems: Journal of Geophysical Research 100, B7, pp. 12431-12447.

\bibitem{MT02} 
Mosegaard, K., and Tarantola, A., 2002: Probabilistic Approach to Inverse Problems: Chapter for the International Handbook of Earthquake and Engineering Seismology p 237-265. (Academic Press, ISBN 0-12-440652-1) Published for the International Association of Seismology and Physics of the Earth Interior (IASPEI).

\bibitem{M06}
Mosegaard, K., 2006: Monte Carlo Analysis of Inverse Problems. Doctoral Thesis, University of Copenhagen, ISBN 87-991228-0-4.



\end{thebibliography}
%%
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
\clearpage

%}%end\small
\renewcommand{\labelenumi}{\theenumi.}
\clearpage

\end{document}


==> 1-MC Inversion Guided by Simplified Physics - Basic Theory/cuts.sync-conflict-20200510-203736-JFKMSGX.tex <==
\item[] Spicer, P. E., Nijhoff, F. W. and van der Kamp, P. H., 2011. \textit{Nonlinearity}, 
\textbf{24}, 2229

\item[] Barthelemy F M and RT Haftka R T 1993 \textit{Structural optimization} \textbf{5} 129

\item[] Buffon G 1777 \textit{Essai d'arithmetique morale}

\item[] Christen J A, and Fox C 2005 \textit{Journal of Computational and Graphical Statistics} \textbf{14:4} 795

\item[] Frangos M, Marzouk Y, Willcox K, and van Bloemen Waanders B 2001 \textit{Computational Methods for Large-Scale Inverse Problems and Quantification of Uncertainty} (John Wiley \& Sons, Ltd) p~123

\item[] Ginting V, Pereira F, Presho M, and Wo S 2011 \textit{Comput Geosci} \textbf{15} 691

\item[] Laloy E, Rogiers B, Vrugt J A, Mallants D, and D. Jacques D 2013 \textit{Water Resources Research} \textbf{49} 2664



==> 1-MC Inversion Guided by Simplified Physics - Basic Theory/cuts.tex <==
\item[] Spicer, P. E., Nijhoff, F. W. and van der Kamp, P. H., 2011. \textit{Nonlinearity}, 
\textbf{24}, 2229

\item[] Barthelemy F M and RT Haftka R T 1993 \textit{Structural optimization} \textbf{5} 129

\item[] Buffon G 1777 \textit{Essai d'arithmetique morale}

\item[] Christen J A, and Fox C 2005 \textit{Journal of Computational and Graphical Statistics} \textbf{14:4} 795

\item[] Frangos M, Marzouk Y, Willcox K, and van Bloemen Waanders B 2001 \textit{Computational Methods for Large-Scale Inverse Problems and Quantification of Uncertainty} (John Wiley \& Sons, Ltd) p~123

\item[] Ginting V, Pereira F, Presho M, and Wo S 2011 \textit{Comput Geosci} \textbf{15} 691

\item[] Laloy E, Rogiers B, Vrugt J A, Mallants D, and D. Jacques D 2013 \textit{Water Resources Research} \textbf{49} 2664

-------------

$^{1}$Department of Physics of Ice, Climate and Earth, Tagensvej 16, 2200 Copenhagen N, Denmark}
% \ead{sarouyeh@nbi.ku.dk

-------------

\bibitem{} Mosegaard K and Tarantola A 1995 \textit{Journal of Geophysical Research 100} \textbf{B7} 12431

\bibitem{} Mosegaard K and Tarantola A 2002 \textit{International Handbook of Earthquake and Engineering Seismology} (Academic Press, ISBN 0-12-440652-1) p~237

\bibitem{} Mosegaard K {Monte Carlo Analysis of Inverse Problems} (Doctoral Thesis, University of Copenhagen, ISBN 87-991228-0-4)

\bibitem{} Wolpert D H and Macready W G 1997 \textit{IEEE Transactions on Evolutionary Computation} \textbf{1} 67

\bibitem{} Yin Y 2005 \textit{Soft Computing} \textbf{9} 3


-----

This leads to rather efficient algorithms based on iterative, linearized inversion, where a limited number of iterations lead to an acceptable solution. 


==> 1-MC Inversion Guided by Simplified Physics - Basic Theory/definitions.tex <==
\usepackage{times}
%\usepackage{mathptm}
%\usepackage{mathpple}
%\usepackage{bookman}
 \usepackage{graphicx}
 \usepackage{makeidx}
 \usepackage{amsmath}
 \usepackage{amssymb}
 \usepackage[mathscr]{eucal}
 %\usepackage{pdfsync}
 
% \textheight  = 225 mm
% \textwidth   = 170 mm
% \hoffset     =  -5 mm
% \voffset     = -23 mm
% \evensidemargin =  0 mm
% \oddsidemargin  =  0 mm

\def \VariableWidthFigure#1#2#3#4#5{
    \begin{figure}[htbp]
    \begin{minipage}[c]{#1}
    \caption{#4}\label{#5} \end{minipage}
    \hfill\begin{minipage}[c]{#2}
    \includegraphics[width=#2]{#3}\end{minipage}
    \end{figure}}

 \def \bfd{{\bf d}}
 \def \bfg{{\bf g}}
 \def \bfk{{\bf k}}
 \def \bfp{{\bf p}}
 \def \bfx{{\bf x}}
 \def \bfy{{\bf y}}
 \def \bfA{{\bf A}}
 \def \bfC{{\bf C}}
 \def \bfX{{\bf X}}
 \def \bflambda{\boldsymbol{\lambda}}
 \def \PointP{{\mathscr{P}}}
 \def \PointQ{{\mathscr{Q}}}
 \def \LinSpaceL{\boldsymbol{\mathsf{L}}}
 \def \calA{{\cal A}}
 \def \calD{{\cal D}}
 \def \calE{{\cal E}}
 \def \calF{{\cal F}}
 \def \calM{{\cal M}}
 \def \calN{{\cal N}}
 \def \calS{{\cal S}}
 \def \flag{\ast}

 \def \absval#1{\left| \ #1 \ \right|}
 \def \norm#1{\Vert \ #1 \ \Vert}

 \def \onehalf{{\frac{1}{2}}}

%%% AT defs %%%%%

\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfd{{\bf d}}
\def\bff{{\bf f}}
\def\bfe{{\bf e}}
\def\bfg{{\bf g}}
\def\bfm{{\bf m}}
\def\bfp{{\bf p}}
\def\bfr{{\bf r}}
\def\bfs{{\bf s}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfC{{\bf C}}
\def\bfD{{\bf D}}
\def\bfF{{\bf F}}
\def\bfG{{\bf G}}
\def\bfH{{\bf H}}
\def\bfI{{\bf I}}
\def\bfJ{{\bf J}}
\def\bfK{{\bf K}}
\def\bfL{{\bf L}}
\def\bfM{{\bf M}}
\def\bfQ{{\bf Q}}
\def\bfS{{\bf S}}
\def\bfU{{\bf U}}
\def\bfV{{\bf V}}
\def\bfX{{\bf X}}
\def\bfW{{\bf W}}
\def\bfZ{{\bf Z}}

\def\bfalpha{\mbox{\boldmath$\alpha$}}
\def\bfbeta{\mbox{\boldmath$\beta$}}
\def\bfgamma{\mbox{\boldmath$\gamma$}}
\def\bfdelta{\mbox{\boldmath$\delta$}}
\def\bfDelta{\mbox{\boldmath$\Delta$}}
\def\bfkappa{\mbox{\boldmath$\kappa$}}
\def\bfrho{\mbox{\boldmath$\rho$}}
\def\bfpsi{\mbox{\boldmath$\psi$}}
\def\bfsigma{\mbox{\boldmath$\sigma$}}
\def\bfvarepsilon{\mbox{\boldmath$\varepsilon$}}
\def\bfstress{{\bfsigma}}
\def\bfstrain{{\bfvarepsilon}}

\def\cte{{\rm cte.}}
\def\onehalf{{1 \over 2}}
\def\obs{{\rm obs}}
\def\calc{{\rm cal}} % <- do not use `cal' (interference with calligraphics)
\def\prior{{\rm prior}}
\def\post{{\rm post}}
\def\dobs{{\bfd_{\obs}}}
\def\dcal{{\bfd_{\cal}}}
\def\mprior{{\bfm_{\prior}}}
\def\mpost{{\widetilde{\bfm}}}
\def\CD{{\bfC_D}}
\def\CDinv{{\bfC_D^{-1}}}
\def\CM{{\bfC_M}}
\def\CMinv{{\bfC_M^{-1}}}
\def\CMpost{{\widetilde{\bfC}_M}}
\def\gm{{\bfg(\bfm)}}
\def\FT{{\bfF^T}}
\def\FTF{{\FT \CDinv \bfF}}
\def\FFT{{\bfF \CM \FT}}
\def\GT{{\bfG^T}}
\def\GTG{{\GT \CDinv \bfG}}
\def\GGT{{\bfG \CM \GT}}
\def\wdhtbff{{\widehat {\bf f}}}
\def\wdhtbfx{{\widehat  \bfx }}
\def\wdhtbfX{{\widehat  \bfx }}
\def\wdhtf{{\widehat f}}
\def\wdhtg{{\widehat g}}
\def\wdhtx{{\widehat x}}
\def\wdhtbfp{{\widehat {\bf p}}}
\def\wdhtbfs{{\widehat {\bf s}}}
\def\wdhtbfS{{\widehat {\bf S}}}
\def\wdhtp{{\widehat p}}
\def\wdhtS{{\widehat S}}
\def\wdhtbfkappa{{\widehat {\bfkappa}}}
\def\wdhtkappa{{\widehat {\kappa}}}
\def\strain{{\varepsilon}}
\def\stress{{\sigma}}
\def\AND{{\sc and}}
\def\OR{{\sc or}}
\def\NOT{{\sc not}}

\def\partialderiv#1#2{{{\partial #1} \over{\partial #2}}}
\def\partialderivsquared#1#2{{{\partial^2 #1} \over{\partial #2^2}}}
\def\div{{\rm div}}
\def\grad{{\bf grad}}
\def\gradient{\widehat{\mbox{\boldmath $\gamma$}}}
\def\jacobian#1#2{\left[\partialderiv{(#1)}{(#2)}\right]}
\def\dualprod#1#2{\langle \ #1 \ , \ #2 \ \rangle}
\def\scalprod#1#2{( \ #1 \ , \ #2 \ )}
\def\scalarprod#1#2{( \ #1 \ , \ #2 \ )}

\def\implies{{\Rightarrow}}
\def\iff{{\Leftrightarrow}}
\def\IFF{{\Longleftrightarrow}}
\def\chvar{{\rightleftharpoons}}
\def\EndOfExample{{\sc[end of example.]}}

\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calI{{\cal I}}
\def\calM{{\cal M}}
\def\calP{{\cal P}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calX{{\cal X}}

\def\ND{{\rm ND}}
\def\NM{{\rm NM}}

\def\({\left(}
\def\){\right)}

\def\begeq{\begin{equation}}
\def\endeq{\end{equation}}
\def\begeqarray{\begin{eqnarray}}
\def\endeqarray{\end{eqnarray}}


%%% end AT defs %%%%%

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % The Newtheorem Context
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

\newtheorem{Example}{Example}%[section]
\newtheorem{Postulate}{Postulate}%[section]
\newtheorem{Lemma}{Lemma}%[section]
\newtheorem{Theorem}{Theorem}%[section]
\newtheorem{Proposition}{Proposition}%[section]
\newtheorem{Corollary}{Corollary}%[section]
\newtheorem{Property}{Property}%[section]
\newtheorem{Conjecture}{Conjecture}%[section]
\newtheorem{Proof}{Proof}%[section]
\newtheorem{Demonstration}{Demonstration}%[section]
\newtheorem{Definition}{Definition}%[section]
\newtheorem{Comment}{Comment}%[section]
\newtheorem{Algorithm}{Algorithm}%[section]

\setcounter{secnumdepth}{0}
\setcounter{tocdepth}{2}


==> 1-MC Inversion Guided by Simplified Physics - Basic Theory/ipdefinitions.tex <==
\usepackage{times}
%\usepackage{mathptm}
%\usepackage{mathpple}
%\usepackage{bookman}
%\usepackage{subcaption}
\usepackage{subfig}
\usepackage{graphicx}
%% \usepackage{makeidx}
%% \usepackage{amsmath}
%% \usepackage{amssymb}
%% \usepackage[mathscr]{eucal}
 %\usepackage{pdfsync}
 
% \textheight  = 225 mm
% \textwidth   = 170 mm
% \hoffset     =  -5 mm
% \voffset     = -23 mm
% \evensidemargin =  0 mm
% \oddsidemargin  =  0 mm

\def \VariableWidthFigure#1#2#3#4#5{
    \begin{figure}[htbp]
    \begin{minipage}[c]{#1}
    \caption{#4}\label{#5} \end{minipage}
    \hfill\begin{minipage}[c]{#2}
    \includegraphics[width=#2]{#3}\end{minipage}
    \end{figure}}

 \def \bfd{{\bf d}}
 \def \bfg{{\bf g}}
 \def \bfk{{\bf k}}
 \def \bfp{{\bf p}}
 \def \bfx{{\bf x}}
 \def \bfy{{\bf y}}
 \def \bfA{{\bf A}}
 \def \bfC{{\bf C}}
 \def \bfX{{\bf X}}
 \def \bflambda{\boldsymbol{\lambda}}
 \def \PointP{{\mathscr{P}}}
 \def \PointQ{{\mathscr{Q}}}
 \def \LinSpaceL{\boldsymbol{\mathsf{L}}}
 \def \calA{{\cal A}}
 \def \calD{{\cal D}}
 \def \calE{{\cal E}}
 \def \calF{{\cal F}}
 \def \calL{{\cal L}}
 \def \calM{{\cal M}}
 \def \calN{{\cal N}}
 \def \calS{{\cal S}}
 \def \flag{\ast}

 \def \absval#1{\left| \ #1 \ \right|}
 \def \norm#1{\Vert \ #1 \ \Vert}

 \def \onehalf{{\frac{1}{2}}}

%%% AT defs %%%%%

\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfd{{\bf d}}
\def\bff{{\bf f}}
\def\bfe{{\bf e}}
\def\bfg{{\bf g}}
\def\bfh{{\bf h}}
\def\bfm{{\bf m}}
\def\bfn{{\bf n}}
\def\bfp{{\bf p}}
\def\bfr{{\bf r}}
\def\bfs{{\bf s}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfz{{\bf z}}
\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfC{{\bf C}}
\def\bfD{{\bf D}}
\def\bfF{{\bf F}}
\def\bfG{{\bf G}}
\def\bfH{{\bf H}}
\def\bfI{{\bf I}}
\def\bfJ{{\bf J}}
\def\bfK{{\bf K}}
\def\bfL{{\bf L}}
\def\bfM{{\bf M}}
\def\bfQ{{\bf Q}}
\def\bfS{{\bf S}}
\def\bfU{{\bf U}}
\def\bfV{{\bf V}}
\def\bfX{{\bf X}}
\def\bfW{{\bf W}}
\def\bfZ{{\bf Z}}

\def\bfalpha{\mbox{\boldmath$\alpha$}}
\def\bfbeta{\mbox{\boldmath$\beta$}}
\def\bfgamma{\mbox{\boldmath$\gamma$}}
\def\bfdelta{\mbox{\boldmath$\delta$}}
\def\bfDelta{\mbox{\boldmath$\Delta$}}
\def\bfkappa{\mbox{\boldmath$\kappa$}}
\def\bfrho{\mbox{\boldmath$\rho$}}
\def\bfpsi{\mbox{\boldmath$\psi$}}
\def\bfsigma{\mbox{\boldmath$\sigma$}}
\def\bfvarepsilon{\mbox{\boldmath$\varepsilon$}}
\def\bfstress{{\bfsigma}}
\def\bfstrain{{\bfvarepsilon}}

\def\cte{{\rm cte.}}
\def\onehalf{{1 \over 2}}
\def\obs{{\rm obs}}
\def\calc{{\rm cal}} % <- do not use `cal' (interference with calligraphics)
\def\prior{{\rm prior}}
\def\post{{\rm post}}
\def\dobs{{\bfd_{\obs}}}
\def\dcal{{\bfd_{\cal}}}
\def\mprior{{\bfm_{\prior}}}
\def\mpost{{\widetilde{\bfm}}}
\def\CD{{\bfC_D}}
\def\CDinv{{\bfC_D^{-1}}}
\def\CM{{\bfC_M}}
\def\CMinv{{\bfC_M^{-1}}}
\def\CMpost{{\widetilde{\bfC}_M}}
\def\gm{{\bfg(\bfm)}}
\def\FT{{\bfF^T}}
\def\FTF{{\FT \CDinv \bfF}}
\def\FFT{{\bfF \CM \FT}}
\def\GT{{\bfG^T}}
\def\GTG{{\GT \CDinv \bfG}}
\def\GGT{{\bfG \CM \GT}}
\def\wdhtbff{{\widehat {\bf f}}}
\def\wdhtbfx{{\widehat  \bfx }}
\def\wdhtbfX{{\widehat  \bfx }}
\def\wdhtf{{\widehat f}}
\def\wdhtg{{\widehat g}}
\def\wdhtx{{\widehat x}}
\def\wdhtbfp{{\widehat {\bf p}}}
\def\wdhtbfs{{\widehat {\bf s}}}
\def\wdhtbfS{{\widehat {\bf S}}}
\def\wdhtp{{\widehat p}}
\def\wdhtS{{\widehat S}}
\def\wdhtbfkappa{{\widehat {\bfkappa}}}
\def\wdhtkappa{{\widehat {\kappa}}}
\def\strain{{\varepsilon}}
\def\stress{{\sigma}}
\def\AND{{\sc and}}
\def\OR{{\sc or}}
\def\NOT{{\sc not}}

\def\partialderiv#1#2{{{\partial #1} \over{\partial #2}}}
\def\partialderivsquared#1#2{{{\partial^2 #1} \over{\partial #2^2}}}
\def\div{{\rm div}}
\def\grad{{\bf grad}}
\def\gradient{\widehat{\mbox{\boldmath $\gamma$}}}
\def\jacobian#1#2{\left[\partialderiv{(#1)}{(#2)}\right]}
\def\dualprod#1#2{\langle \ #1 \ , \ #2 \ \rangle}
\def\scalprod#1#2{( \ #1 \ , \ #2 \ )}
\def\scalarprod#1#2{( \ #1 \ , \ #2 \ )}

\def\implies{{\Rightarrow}}
\def\iff{{\Leftrightarrow}}
\def\IFF{{\Longleftrightarrow}}
\def\chvar{{\rightleftharpoons}}
\def\EndOfExample{{\sc[end of example.]}}

\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calI{{\cal I}}
\def\calM{{\cal M}}
\def\calP{{\cal P}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calX{{\cal X}}

\def\ND{{\rm ND}}
\def\NM{{\rm NM}}

\def\({\left(}
\def\){\right)}

%\def\begeq{\begin{equation}}
%\def\endeq{\end{equation}}
\def\begeqarray{\begin{eqnarray}}
\def\endeqarray{\end{eqnarray}}


%%% end AT defs %%%%%

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % The Newtheorem Context
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

\newtheorem{Example}{Example}%[section]
\newtheorem{Postulate}{Postulate}%[section]
\newtheorem{Lemma}{Lemma}%[section]
\newtheorem{Theorem}{Theorem}%[section]
\newtheorem{Proposition}{Proposition}%[section]
\newtheorem{Corollary}{Corollary}%[section]
\newtheorem{Property}{Property}%[section]
\newtheorem{Conjecture}{Conjecture}%[section]
\newtheorem{Proof}{Proof}%[section]
\newtheorem{Demonstration}{Demonstration}%[section]
\newtheorem{Definition}{Definition}%[section]
\newtheorem{Comment}{Comment}%[section]
\newtheorem{Algorithm}{Algorithm}%[section]
\newtheorem{Procedure}{Procedure}%[section]

\setcounter{secnumdepth}{1}
\setcounter{tocdepth}{2}


==> MC-with-Phys-Proposals-170919.tex <==
\input{preample.tex}

\begin{document} 
\title{\bf Monte Carlo Sampling with\\ Problem-dependent Proposals}
%\date{ } 

%\thispagestyle{empty}
%\vspace*{10mm}
%\bigskip
\author{Klaus Mosegaard${}^{1}$ \\ Sarouyeh Khoshkholgh${}^{1}$ \\ Others ?$\dots$}
\date{}
\maketitle

{\begin{center}
{${}^1$ Department of Physics of Ice, Climate and Earth, Tagensvej 16, 2200 Copenhagen N, Denmark}
\end{center}
%\vspace*{2mm}
%\begin{center}
%{${}^2$Department of Earth Sciences \\ ETH Zuerich,
%Sonneggstrasse 5, 8092 Zuerich Switzerland} 
%\vspace*{10mm}
%%\\ {Klaus Mosegaard  \\  2004}
%\end{center}
}

\setcounter{page}{0}

%
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
%\clearpage
%
%\tableofcontents
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
%\clearpage

\begin{abstract}
Abstract abstract abstract abstract abstract abstract abstract abstract 
\end{abstract}

\section{Introduction}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
Introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction introduction  
 
\section{Classical MCMC}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
In this section we follow Tarantola and Valette (1982a) whose formulation of the probabilistic inference problem is based on an expression for the conjunction of information given by two probability densities $f_1(\bfx)$ and $f_2(\bfx)$ over the same space $\calX$:
$$
(f_1 \wedge f_2) (\bfx) = \frac{f_1(\bfx) f_2(\bfx)}{\mu(\bfx)}.
$$ 
where ${\mu(\bfx)}$ is the homogeneous probability density assigning equal probabilities to equal volumes in $\calX$.
They adapt this formula to the inference problem by defining $\bfx = (\bfd,\bfm)$ as a point in the joint data-model space, and obtain the posterior probability distribution:
$$
\sigma(\bfd,\bfm) = \frac{\rho(\bfd,\bfm) \theta(\bfd,\bfm)}{\mu(\bfd,\bfm)}.
$$
Under the assumption that the priors over $\bfd$ and $\bfm$ are independent, that is, $\rho(\bfd,\bfm)=\rho_d(\bfd) \rho_m(\bfm)$, that $\mu(\bfd,\bfm)$ is constant, and that the physical relation $\bfd = \bfg(\bfm)$ is exact, such that $\theta(\bfd,\bfm)=\delta(\bfd - \bfg(\bfm)) \mu(\bfm)$, we arrive at an expression for the posterior in the model space
\begin{equation}
\sigma_m(\bfm) = L(\bfm)\rho_m(\bfm)
\label{TV-Bayes}
\end{equation} 
with
$L(\bfm)=\rho_d(\bfg(\bfm)).$
Equation (\ref{TV-Bayes}) is equivalent to the classical Bayes Formula, which in our notation reads
$$
\sigma_m(\bfm | \bfd) = \frac{L(\bfd | \bfm)\rho_m(\bfm)}{\rho_d(\bfd)}.
$$
The posterior distribution (\ref{TV-Bayes}) is generally impossible to calculate directly, except for linear inverse problems, so one has to rely on Monte Carlo sampling methods to generate realizations from the distribution. A commonly used approach is the Extended Metropolis Algorithm (\cite{MT95,M06}):

\bigskip\noindent
\begin{Algorithm}
\label{algo: ext-Metro}
\textbf{(Extended Metropolis).} Given a random algorithm $V\left( \mathbf{m}\right) 
$ which iteratively samples the prior probability density ${\rho_m (\mathbf{m})}$: 
\begin{equation}
\mathbf{m}^{(n+1)}=V\left( \mathbf{m}^{(n)}\right) ,  \label{eq: priorwalk}
\end{equation}
and an algoritm $U\left( 0,1\right) $ producing random numbers from the interval $\left[ 0,1\right]$ with uniform probability. The random algorithm $W$, which iteratively updates the current parameter vector $\mathbf{m}^{(n)}$: 
\begin{equation}
\mathbf{m}^{(n+1)}=W\left( \mathbf{m}^{(n)}\right) =\left\{ 
\begin{array}{l}
V\left( \mathbf{m}^{(n)}\right) \text{ if }U\left( 0,1\right) \leq \min
\left[ 1,\frac{L\left( V\left( \mathbf{m}^{(n)}\right) \right) }{L\left( 
\mathbf{m}^{(n)}\right) }\right]  \\ 
\mathbf{m}^{(n)}\text{ else}
\end{array}
,\right.   \label{bigwalk}
\end{equation}
will asymptotically sample the posterior ${\sigma (\mathbf{m}) \propto L(\mathbf{m})\rho (%
\mathbf{m})}$.
\end{Algorithm}

\bigskip\noindent
Algorithm~\ref{algo: ext-Metro} works if the prior sampler $V$ is {\em irreducible} and {\em aperiodic} (see, e.g., \cite{MT02}). 

\bigskip\noindent
The extended Metropolis will, in general, perform better than a regular Metropolis, since only models that are accepted a priori (by $V$) will be subject to the time consuming misfit calculation needed to evaluate $L({\bf m}) $.

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
\section{No-Free-Lunch Theorems and the importance of information}
\label{sec:NFL}
Text text text text text text text text text text text text text  


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%
\section{Blind and Informed Proposals Mechanisms}
Despite the improved efficiency of Algorithm (\ref{algo: ext-Metro}) gained from the use of a prior sampler $V$ in the initial phase of each algorithm, practical experience shows that the efficiency of extended Metropolis is highly dependent on the choice of $V$. The problem is that the prior $\rho$ and the likelihood function $L$ are usually so different that the moves in the model space proposed by $V$ will usually lead to points with low values of $L$. As explained earlier, there is little hope that even the best, blind sampling strategy will be able to significantly improve on this problem. In the following we shall therefore describe a method that will allow us to inject information about the physical relation between data and model parameters into the sampling strategy. First, however, we will understand why the 'blind' strategy of the classical MCMC is so inefficient.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Proposal Distributions in Classical MCMC}
The basic idea behind any implementation of the Metropolis Algorithm is an interplay between {\em proposals} and {\em rejections}. In each iteration, sampling from a probability density $f(\bfx)$ over a space $\calX$ proceeds from a current value $\bfx$ by first proposing a new value ${\bfx}'$ from the so-called {\em proposal distribution} $q({\bfx}',\bfx)$, followed by a random decision where ${\bfx}'$ is accepted with probability
%
\begin{equation}
P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}={\rm min} \( \frac{f({\bfx}') q(\bfx|{\bfx}')}{f(\bfx) q({\bfx}'|\bfx)},1 \).
\end{equation}
%
This follows from the requirement that the probability that a transition takes place from $\bfx$ to ${\bfx}'$, namely
$P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'} q({\bfx}'|\bfx) f(\bfx)$, must be equal to the probability of the reverse transition
$P_{\rm acc}^{{\bfx}' \rightarrow {\bfx}} q(\bfx|{\bfx}') f({\bfx}')$ to attain equilibrium sampling (detailed balance). At this point it is important to note that the proposal distribution has no influence on the distribution to which the sampling converges, it only influences the speed of convergence. 

It is common practice (but not a necessity) to work with symmetric proposal distributions: $q({\bfx}',\bfx) = q(\bfx , {\bfx})$, and in this case we get the simpler expression
\begin{equation}
P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}={\rm min} \( \frac{f({\bfx}')}{f(\bfx)},1 \).
\label{eq_accept}
\end{equation}
%
The Metropolis sampler is only efficient if large enough steps (to connect any two high value areas of $f(\bfx)$ in a few steps) will be frequently accepted. This ability critically depends on the $q({\bfx}',\bfx)$, and that is reason why intensive research in recent years has been devoted to finding improved proposal distributions. 

A close look at the expression for the unconditional transition probability from $\bfx$ to $\bfx'$ (for symmetric $q$)
\begin{equation}
P^{{\bfx} \rightarrow {\bfx}'}=f(\bfx) P_{\rm acc}^{{\bfx} \rightarrow {\bfx}'}=f(\bfx) \cdot q({\bfx}'|\bfx) \cdot {\rm min} \( \frac{f({\bfx}')}{f(\bfx)},1 \).
\end{equation}
shows that, if $f(\bfx)'$ turns out to be low  in places where $q({\bfx}'|\bfx)$ is high, the move ${\bfx} \rightarrow {\bfx}'$ is very likely to be rejected. 

To investigate and exemplify the importance of this problem in high-dimension\-al spaces, let us consider the case where the distribution of ${\bfx}$ is Gaussian with covariance matrix $\bfC$ and mean $\bfx_0$:
$f({\bfx}) = \calN_{\bfx} (\bfx_0,\bfC)$.
Assume now that out proposal distribution is an isotropic Gaussian $q({\bfx}|{\bfx}_q) = \calN_{\bfx} (\bfx_q,\bfC_q)$ with mean ${\bfx}_q$ and covariance matrix $\bfC_q$, 
and that we, in the sampling process, have arrived at point with a high value of $f({\bfx})$, say, for simplicity, at its maximum point ${\bfx}_0$. We can now calculate the expected acceptance probability $P^{{\bfx}_0 \rightarrow {\bfx}}$ proposed in the next step by the algorithm:
\begin{align}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) 
&= \int_{\calX} \frac{f({\bfx})}{f({\bfx}_0)} q({\bfx}|{\bfx}_0) d{\bfx} \label{eq: Meanf1} \\
&= \int_{\calX} \frac{\calN_{\bfx} (\bfx_0,\bfC)}{\calN_{\bfx_0} (\bfx_0,\bfC)} \calN_{\bfx} (\bfx_0,\bfC_q) d{\bfx} \\
&= \frac{\calN_{\bfx_0} (\bfx_0,\bfC+\bfC_q)}{\calN_{\bfx_0} (\bfx_0,\bfC)}\int_{\calX} 
\calN_{\bfx} (\bfx_1,\bfC_1) d{\bfx} 
\label{eq: Meanf}
\end{align}
where
\begin{equation*}
\bfx_1 
= (\bfC^{-1} + \bfC_q^{-1})^{-1} (\bfC^{-1} \bfx_0 + \bfC_q^{-1} \bfx_0) = \bfx_0
\end{equation*}
and 
\begin{equation*}
\bfC_1 = (\bfC^{-1} + \bfC_q^{-1})^{-1} \, .
\end{equation*}
Since the integral in (\ref{eq: Meanf}) is $1$, we have the following expression for the expected acceptance probability:
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) = \frac{\calN_{\bfx_0} (\bfx_0,\bfC+\bfC_q)}{\calN_{\bfx_0} (\bfx_0,\bfC)} 
= \( \frac{{\rm det}\( 2\pi \bfC \)}{{\rm det}\( 2\pi (\bfC+\bfC_q) \)} \)^{1/2} \, .
\end{equation}
Both $\bfC_q = \sigma_q^2 {\bfI}$ (with $\sigma_q^2 > 0$) and $\bfC$ are diagonal in the frame spanned by $\bfC$'s eigenvectors, and if we assume that the eigenvalues of $\bfC$ are $\sigma_1^2 \ge \dots \ge \sigma_N^2 > 0$, where $N$ is the dimension of $\calX$, the eigenvalues of $\bfC+\bfC_q$ are
$(\sigma_1^2+\sigma_q^2), \dots ,(\sigma_N^2+\sigma_q^2)$. From this we have  
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) = \prod_{n=1}^N
\( \frac{\sigma_n^2}{\sigma_n^2+\sigma_q^2}
\)^{1/2} \, .
\label{eq-eigenC1}
\end{equation}
From (\ref{eq-eigenC1}) we see that for any non-zero values of $\sigma_n$ and $\sigma_q$ we have 
\begin{equation}
E(P^{{\bfx}_0 \rightarrow {\bfx}}) \rightarrow 0 \quad {\rm for} \quad N \rightarrow  \infty \, .
\end{equation}
expressing the influence on sampling of the so-called 'curse of dimensionality'. If the proposed steps are kept very short ($\sigma_q$ is small compared to all $\sigma_n$), the decrease of $E(P^{{\bfx}_0 \rightarrow {\bfx}})$ with $N$ is slow. But this situation is of no practical value, because adequate sampling by the algorithm requires that it can traverse high-probability areas of $f({\bfx})$ within a reasonable amount of time. 

For non-negligible step lengths, the situation is radically different. Indeed, if there exists an integer $K$ and a real constant $k$ such that $\sigma_q > k\sigma_n$ for all $n > K$, then $E(P^{{\bfx}_0 \rightarrow {\bfx}})$ decreases more that exponentially with $N$. In other words, if the distribution $f({\bfx})$ is 'elongated' compared to the proposal $q$, that is, if it is broader than $q$ in only a finite number of directions/dimensions, the mean number of accepted moves will decrease at least exponentially with the number of dimensions.

As an example, let us consider the case where $\sigma_q^2 = 1$, and $\sigma_n^2 = 1/n$. For $N=2$ this gives an expected acceptance probability of $0.4082$, corresponding to a mean waiting time of about $0.4082^{-1} \approx 2.5$ iterations between accepted moves. For $N=10$ the expectation is $1.5828 \cdot 10^{-4}$, and for $N=100$ it decreases to $1.03 \cdot 10^{-80}$, giving a waiting time of about $3.0 \cdot 10^{62}$ years for 1 Billion iterations per second.

The above analysis is carried out under the very favourable situation where the maximum of $f({\bfx})$ has been located by the algorithm, and does not even consider the serious difficulties faced by the sampling algorithm in the initial search for points with high values of $f({\bfx})$ (the {\em burn in} phase). So it is clear that the proposal mechanism, as defined by $q$, is the Achilles heel of the standard MCMC approach.
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% Section
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Sampling with Problem-dependent Proposals}
The unsurmountable difficulties described in the previous section are rooted in the fact that standard MCMC calculations are essentially blind search algorithms supplemented with a few problem-specific features. To evade the fundamental problems of classical MCMC sampling, we shall therefore take the consequence of the legacy of the No-Free-Lunch theorem and propose a class of algorithms that explicitly incorporates information about the problem to be solved.

To avoid a mismatch between the distribution $f({\bfx})$ to be sampled, and the proposal distribution $q(\bfx' | \bfx)$, we shall in the following look into proposals $q$ that are approximations to $f$, in the sense that 
\begin{equation}
q(\bfx' | \bfx) = \tilde{f} ({\bfx'})
\end{equation}
where the Kullbach-Leibler divergence
\begin{equation}
D(f,\tilde{f}) = \int_\calX f({\bfx}) \log \( \frac{f({\bfx})}{\tilde{f}(\bfx)} \) d{\bfx}
\end{equation}
is small. For a given inverse problem, the challenge is here to derive $\tilde{f}({\bfx})$. We shall devote the next section to this problem, where the focus will be on the special conditions characterizing inverse problems. 

\subsection{Inverse Problems: proposing through approximate forwards} 
When applying an MCMC method to inverse problems, where $f(\bfx)$ is the posterior $\sigma(\bfx)$ or the likelihood $L(\bfx)$, the expected acceptance probability is given by (\ref{eq: Meanf1}). This expression is largest (equal to $1$) when $f({\bfx}_0) = q({\bfx}|{\bfx}_0)$ for all $\bfx$, or, when $q$ is symmetric, $f({\bfx}) = q({\bfx}|{\bfx}_0)$ for all $\bfx_0$. In case $q({\bfx}|{\bfx}_0)$ deviates from $f(\bfx)$ there will be areas within $\calX$ where $q({\bfx}|{\bfx}_0)<f(\bfx)$ as well as areas with  $q({\bfx}|{\bfx}_0)>f(\bfx)$, because both $f$ and $q({\bfx}|{\bfx}_0)$ are positive with integral $1$ over $\calX$. It is, however, the areas with $q({\bfx}|{\bfx}_0)<f(\bfx)$ that are critical, because they directly reduce the acceptance probability. In the following we exploit this fact to construct approximate likelihood functions or posterior distributions, allowing efficient sampling of solutions to inverse problems.

\subsubsection{Approximate posteriors}
Consider an inverse problem with observational data $\bfd^{obs}$ and computed data 
\begin{equation*}
{\bfd} = {\bfg}({\bfm}) \, .
\end{equation*}
Here, ${\bfg}$ is an exact forward function. Suppose that we also have an approximate forward relation $\tilde{\bfg}$ that allows us efficiently compute approximate data
\begin{equation*}
\tilde{\bfd} = \tilde{\bfg}({\bfm}) \, .
\end{equation*}
and that a (possibly simplified) prior probability density 
$\tilde{\rho}_m({\bfm})$ is available.  With this method in hand we can form an approximate posterior probability distribution
\begin{equation}
\tilde{\sigma}({\bfm}) = \tilde{L}({\bfm}) \tilde{\rho}_m({\bfm}) = \rho_d (\tilde{\bfg}({\bfm})) \tilde{\rho}_m({\bfm})
\end{equation}
which can be used directly as a proposal distribution: 
\begin{equation}
q({\bfm}'|{\bfm}) = \tilde{\sigma}({\bfm}') \, .
\end{equation}
Another approach is to use some 'pseudo-inverse' function 
$\bfh$ (if available) on the observed data $\bfd_{obs}$:
\begin{equation*}
{\bfm}_{est} = {\bfh}(\bfd_{obs}) \, .
\end{equation*}
and to use the image $\sigma_{pseud}$ of the data distribution $\rho_d$ under $\bfh$:
\begin{equation}
\sigma_{pseud}({\bfm})
 = 
\frac{\partial{\tilde{\bfh}}}{\partial{\bfd}}\rho_d({\bfd}) \, .
\end{equation}
as a proposal distribution
\begin{equation}
q({\bfm}'|{\bfm}) = \sigma_{pseud}({\bfm}') \, .
\end{equation}
However, the fact that we can use the above approximations to the posterior as proposals does not mean that they are efficient. In the following sections we shall analyse some necessary conditions for efficiency, and give examples of implementations. The efficiency conditions will, of course, depend on the category of problems we face (linear, mildly non-linear, highly non-linear), so we will consider these situations in turn.

\subsubsection{Linear, Gaussian Problems}
Sampling of solutions to a linear Gaussian problem through rejection sampling is straightforward. We have an explicit expression for the Gaussian posterior, and the distribution itself can be used as an exact proposal. Samples $\bfm$ from an $N$-dimensional standard (isotropic) Gaussian (mean $\bf 0$ and covariance $\bfI$) can be generated with the Box-M\"uller method, and the desired samples ${\bfm}$ from a $N$-dimensional multivariate Gaussian with mean ${\bfm}_0$ and covariance $\bfC$ can be calculated as 
${\bfm} ={\bfm}_0 + {\bfA}{\bfm}$, 
where ${\bfA}{\bfA}^T = {\bfC}$. The matrix ${\bfA}$ can be found by, for instance, Cholesky decomposition.

\subsubsection{Nonlinear Problems}
We shall now propose a procedure for efficient sampling of solutions to nonlinear problems with a homogeneous (constant) prior. 

\medskip
\noindent
Given an inverse problem 
\begin{equation*}
{\bfd} = {\bfg}({\bfm})
\end{equation*}
with homogeneous prior, observed data ${\bfd}_{obs}$, and data covariance matrix $\bfC_d$. The problem is characterized by its likelihood function
$L({\bfm}) = \calN_{\bfd_{obs}}({\bfg}({\bfm}),{\bfC}_d)$. 
and its prior $\rho(\bfm) = \mu(\bfm)$, and will in the following be expressed through the notation
\begin{equation}
\calP = \{ \calN_{\bfd_{obs}}({\bfg}({\bfm}),{\bfC}_d), \mu(\bfm) \} \, .
\end{equation}
We shall furthermore consider an approximation to $\calP$
\begin{equation}
\tilde{\calP} = \{ \calN_{\bfd_{obs}}(\tilde{\bfg}({\bfm}),{\bfC}_d), \mu(\bfm) \} \, ,
\end{equation}
As a measure of the difference between the exact posterior and the approximate posterior in the joint $(\bfd,\bfm)$-space, we shall use the Kullbach-Leibler divergence of the conditional $\sigma(\bfd |\bfm)$:
\begin{align}
D(\sigma(\bfd |\bfm),\tilde{\sigma}(\bfd |\bfm)) 
&= \int_\calX \sigma({\bfd}|{\bfm}) \log \( \frac{\sigma({\bfd}|{\bfm})}{\tilde{\sigma}({\bfd}|\bfm)} \) d{\bfd} \label{eq: Kull} \\
&= \int_\calX \calN_{\bfd}({\bfg}({\bfm}),{\bfC}_d) \log \( \frac{\calN_{\bfd}({\bfg}({\bfm}),{\bfC}_d)}{\calN_{\bfd}(\tilde{\bfg}({\bfm}),{\bfC}_d)} \) d{\bfd} \\
&= \frac{1}{2} \({\bfg}({\bfm})-\tilde{\bfg}({\bfm}))^T {\bfC}_d^{-1} ({\bfg}({\bfm})-\tilde{\bfg}({\bfm})) \) \\
&= \frac{1}{2} \| {\bfg}({\bfm})-\tilde{\bfg}({\bfm}) \|_{{\bfC}_d}^2
\end{align}
which is the ${\calL}_2$-distance with weight matrix ${\bfC}_d$ between the approximate, computed data $\tilde{\bfg}({\bfm})$ and the exact, computed data ${\bfg}({\bfm})$. This shows that the amount of information missing in $\tilde{\calP}$, compared to $\calP$ (the Kullbach-Leibler divergence) can be measured directly from the difference between ${\bfg}({\bfm})$ and $\tilde{\bfg}({\bfm})$.



\medskip\noindent
This suggests the following:
\noindent
\begin{Algorithm}
Use $\calN_{\bfd_{obs}}(\tilde{\bfg}({\bfm}),{\bfC}_d)$ as the proposal distribution in Algoritm (\ref{algo: ext-Metro}).
\label{algo: ext-Metro-KBMC}
\end{Algorithm}

\subsubsection{Example: A 100-parameter inverse scattering problem}
Figure $\dots$ shows acoustic impedances of a 1000-parameter, horizontally stratified earth model, and the vertical-incidence seismic data generated from the model. The data are 1D full-waveform seismic signals, generated and recorded at the surface. The full-waveform data contains all multiple reflections, transmission losses and damping effects, so the inverse problem of recovering the model from the data is highly nonlinear. A linearized approximate solution to the inverse scattering problem (in the absence of noise) is shown to the right. This solution requires very little computation time, but is clearly inaccurate (compare to left graph). A more accurate solution, with uncertainty estimates, can be obtained by Markov chain Monte Carlo (MCMC) if enough samples can be obtained in reasonable time. Figure  $\dots$ (upper curve) shows the lack of convergence to equilibrium of a classical MCMC in the first 2000 iterations of such an inversion process. The lower curve, however, shows much faster convergence of a Algorithm (\ref{algo: ext-Metro-KBMC}) whose random walk is guided by the linearized solution shown in Figure $\dots$. Algorithm (\ref{algo: ext-Metro-KBMC}) uses a forward modeling error distribution centered in the linearized solution to choose samples. The improvement in convergence time is dramatic, in this case of the order of $10^4$ when started at the same model as the Algorithm (\ref{algo: ext-Metro}).


%\begin{figure}[htp]
%
%  \centering
%
%  \label{figur}
%
%  \begin{tabular}{cc}
%
%    % Requires \usepackage{graphicx}
%
%    \framebox{\includegraphics[width=1.8in]{TrueModel-xx.png}}
%    \framebox{\includegraphics[width=1.01in]{dobs.png}}
%    \framebox{\includegraphics[width=1.8in]{ApproxModel.png}} \\
%    
%  \end{tabular}
%  \caption{A 1000-layer, horizontally stratified Earth model (left), the corresponding vertical-incidence, full-waveform seismic data (middle), and a classical, linearized solution to the inverse problem (right).}
%\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{TrueModel-xx.png}
        %\caption{A gull}
        %\label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{dobs.png}
        %\caption{A tiger}
        %\label{fig:tiger}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{ApproxModel.png}
        %\caption{A mouse}
        %\label{fig:mouse}
    \end{subfigure}
    \caption{A 1000-layer, horizontally stratified Earth model (left), the corresponding vertical-incidence, full-waveform seismic data (middle), and a classical, linearized solution to the inverse problem (right).}\label{fig:animals}
\end{figure}



\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{Exp-1-Iter-10000-TrueErrorEnvelope.png}
\caption{Linear Inversion: Modelization Error: True Error Envelope} 
\end{center}
\end{figure}

\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{Exp-1-Iter-10000-EstErrorEnvelope.png}
\caption{Linear Inversion: Modelization Error: Est Error Envelope} 
\end{center}
\end{figure}

\vfill

\begin{figure}[h]
%\label{fig-mitera}
\begin{center}
\includegraphics[width=4in]{IMC-MCMC-iter-2000-Misfits-x.png}
\caption{Convergence towards equilibrium of a classical MCMC algorithm (upper curve), attempting to sample solutions to the inverse problem described in Figure 5. Lower curve is the fast-converging KBMC algorithm guided by the linearized inversion. In this case the convergence of the KBMC algorithm was of the order of 104 times faster than the MCMC algorithm.} 
\end{center}
\end{figure}

\vfill

%We will improve algorithm performance by introducing the concept of passive prior information (contrast to usual active prior information used in Bayes Rule). Passive priors carry simplified information about relations between data and unknown model parameters to improve algorithmic convergence, but do not influence the posterior distribution directly. Passive priors can be built from neural networks, simplified physics, or other representations of relations in Nature.



%\vskip 1.5cm
\medskip
\noindent
%
%
%
%\newpage
\subsubsection{Procedure 2: Sampling with General Prior}
({\dots soon to appear\dots)



%\thispagestyle{empty}
%\vspace*{60mm}
\clearpage


%\section{References}

\newcommand{\marginlabel}[1]
   {\mbox{}\marginpar{\raggedleft\hspace{0pt}#1}}

\begin{thebibliography}{999}

%\bibitem{B1773}
%Buffon, G., Memoire sur le jeu de franc-carreau, 1733

%\reversemarginpar

\bibitem{B1777}
Buffon, G., 1777. Essai d'arithmetique morale.

\bibitem{MT95} 
Mosegaard, K., and Tarantola, A., 1995. Monte Carlo sampling of solutions to inverse problems: Journal of Geophysical Research 100, B7, pp. 12431-12447.

\bibitem{MT02} 
Mosegaard, K., and Tarantola, A., 2002: Probabilistic Approach to Inverse Problems: Chapter for the International Handbook of Earthquake and Engineering Seismology p 237-265. (Academic Press, ISBN 0-12-440652-1) Published for the International Association of Seismology and Physics of the Earth Interior (IASPEI).

\bibitem{M06}
Mosegaard, K., 2006: Monte Carlo Analysis of Inverse Problems. Doctoral Thesis, University of Copenhagen, ISBN 87-991228-0-4.



\end{thebibliography}
%%
%\newpage
%\thispagestyle{empty}
%\text{}
%\pagebreak
\clearpage

%}%end\small
\renewcommand{\labelenumi}{\theenumi.}
\clearpage

\end{document}


==> cuts.sync-conflict-20200510-203736-JFKMSGX.tex <==
\item[] Spicer, P. E., Nijhoff, F. W. and van der Kamp, P. H., 2011. \textit{Nonlinearity}, 
\textbf{24}, 2229

\item[] Barthelemy F M and RT Haftka R T 1993 \textit{Structural optimization} \textbf{5} 129

\item[] Buffon G 1777 \textit{Essai d'arithmetique morale}

\item[] Christen J A, and Fox C 2005 \textit{Journal of Computational and Graphical Statistics} \textbf{14:4} 795

\item[] Frangos M, Marzouk Y, Willcox K, and van Bloemen Waanders B 2001 \textit{Computational Methods for Large-Scale Inverse Problems and Quantification of Uncertainty} (John Wiley \& Sons, Ltd) p~123

\item[] Ginting V, Pereira F, Presho M, and Wo S 2011 \textit{Comput Geosci} \textbf{15} 691

\item[] Laloy E, Rogiers B, Vrugt J A, Mallants D, and D. Jacques D 2013 \textit{Water Resources Research} \textbf{49} 2664



==> cuts.tex <==
\item[] Spicer, P. E., Nijhoff, F. W. and van der Kamp, P. H., 2011. \textit{Nonlinearity}, 
\textbf{24}, 2229

\item[] Barthelemy F M and RT Haftka R T 1993 \textit{Structural optimization} \textbf{5} 129

\item[] Buffon G 1777 \textit{Essai d'arithmetique morale}

\item[] Christen J A, and Fox C 2005 \textit{Journal of Computational and Graphical Statistics} \textbf{14:4} 795

\item[] Frangos M, Marzouk Y, Willcox K, and van Bloemen Waanders B 2001 \textit{Computational Methods for Large-Scale Inverse Problems and Quantification of Uncertainty} (John Wiley \& Sons, Ltd) p~123

\item[] Ginting V, Pereira F, Presho M, and Wo S 2011 \textit{Comput Geosci} \textbf{15} 691

\item[] Laloy E, Rogiers B, Vrugt J A, Mallants D, and D. Jacques D 2013 \textit{Water Resources Research} \textbf{49} 2664

-------------

$^{1}$Department of Physics of Ice, Climate and Earth, Tagensvej 16, 2200 Copenhagen N, Denmark}
% \ead{sarouyeh@nbi.ku.dk

-------------

\bibitem{} Mosegaard K and Tarantola A 1995 \textit{Journal of Geophysical Research 100} \textbf{B7} 12431

\bibitem{} Mosegaard K and Tarantola A 2002 \textit{International Handbook of Earthquake and Engineering Seismology} (Academic Press, ISBN 0-12-440652-1) p~237

\bibitem{} Mosegaard K {Monte Carlo Analysis of Inverse Problems} (Doctoral Thesis, University of Copenhagen, ISBN 87-991228-0-4)

\bibitem{} Wolpert D H and Macready W G 1997 \textit{IEEE Transactions on Evolutionary Computation} \textbf{1} 67

\bibitem{} Yin Y 2005 \textit{Soft Computing} \textbf{9} 3


-----

This leads to rather efficient algorithms based on iterative, linearized inversion, where a limited number of iterations lead to an acceptable solution. 


==> ipdefinitions.tex <==
\usepackage{times}
%\usepackage{mathptm}
%\usepackage{mathpple}
%\usepackage{bookman}
%\usepackage{subcaption}
\usepackage{subfig}
\usepackage{graphicx}
%% \usepackage{makeidx}
%% \usepackage{amsmath}
%% \usepackage{amssymb}
%% \usepackage[mathscr]{eucal}
 %\usepackage{pdfsync}
 
% \textheight  = 225 mm
% \textwidth   = 170 mm
% \hoffset     =  -5 mm
% \voffset     = -23 mm
% \evensidemargin =  0 mm
% \oddsidemargin  =  0 mm

\def \VariableWidthFigure#1#2#3#4#5{
    \begin{figure}[htbp]
    \begin{minipage}[c]{#1}
    \caption{#4}\label{#5} \end{minipage}
    \hfill\begin{minipage}[c]{#2}
    \includegraphics[width=#2]{#3}\end{minipage}
    \end{figure}}

 \def \bfd{{\bf d}}
 \def \bfg{{\bf g}}
 \def \bfk{{\bf k}}
 \def \bfp{{\bf p}}
 \def \bfx{{\bf x}}
 \def \bfy{{\bf y}}
 \def \bfA{{\bf A}}
 \def \bfC{{\bf C}}
 \def \bfX{{\bf X}}
 \def \bflambda{\boldsymbol{\lambda}}
 \def \PointP{{\mathscr{P}}}
 \def \PointQ{{\mathscr{Q}}}
 \def \LinSpaceL{\boldsymbol{\mathsf{L}}}
 \def \calA{{\cal A}}
 \def \calD{{\cal D}}
 \def \calE{{\cal E}}
 \def \calF{{\cal F}}
 \def \calL{{\cal L}}
 \def \calM{{\cal M}}
 \def \calN{{\cal N}}
 \def \calS{{\cal S}}
 \def \flag{\ast}

 \def \absval#1{\left| \ #1 \ \right|}
 \def \norm#1{\Vert \ #1 \ \Vert}

 \def \onehalf{{\frac{1}{2}}}

%%% AT defs %%%%%

\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfd{{\bf d}}
\def\bff{{\bf f}}
\def\bfe{{\bf e}}
\def\bfg{{\bf g}}
\def\bfh{{\bf h}}
\def\bfm{{\bf m}}
\def\bfn{{\bf n}}
\def\bfp{{\bf p}}
\def\bfr{{\bf r}}
\def\bfs{{\bf s}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfz{{\bf z}}
\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfC{{\bf C}}
\def\bfD{{\bf D}}
\def\bfF{{\bf F}}
\def\bfG{{\bf G}}
\def\bfH{{\bf H}}
\def\bfI{{\bf I}}
\def\bfJ{{\bf J}}
\def\bfK{{\bf K}}
\def\bfL{{\bf L}}
\def\bfM{{\bf M}}
\def\bfQ{{\bf Q}}
\def\bfS{{\bf S}}
\def\bfU{{\bf U}}
\def\bfV{{\bf V}}
\def\bfX{{\bf X}}
\def\bfW{{\bf W}}
\def\bfZ{{\bf Z}}

\def\bfalpha{\mbox{\boldmath$\alpha$}}
\def\bfbeta{\mbox{\boldmath$\beta$}}
\def\bfgamma{\mbox{\boldmath$\gamma$}}
\def\bfdelta{\mbox{\boldmath$\delta$}}
\def\bfDelta{\mbox{\boldmath$\Delta$}}
\def\bfkappa{\mbox{\boldmath$\kappa$}}
\def\bfrho{\mbox{\boldmath$\rho$}}
\def\bfpsi{\mbox{\boldmath$\psi$}}
\def\bfsigma{\mbox{\boldmath$\sigma$}}
\def\bfvarepsilon{\mbox{\boldmath$\varepsilon$}}
\def\bfstress{{\bfsigma}}
\def\bfstrain{{\bfvarepsilon}}

\def\cte{{\rm cte.}}
\def\onehalf{{1 \over 2}}
\def\obs{{\rm obs}}
\def\calc{{\rm cal}} % <- do not use `cal' (interference with calligraphics)
\def\prior{{\rm prior}}
\def\post{{\rm post}}
\def\dobs{{\bfd_{\obs}}}
\def\dcal{{\bfd_{\cal}}}
\def\mprior{{\bfm_{\prior}}}
\def\mpost{{\widetilde{\bfm}}}
\def\CD{{\bfC_D}}
\def\CDinv{{\bfC_D^{-1}}}
\def\CM{{\bfC_M}}
\def\CMinv{{\bfC_M^{-1}}}
\def\CMpost{{\widetilde{\bfC}_M}}
\def\gm{{\bfg(\bfm)}}
\def\FT{{\bfF^T}}
\def\FTF{{\FT \CDinv \bfF}}
\def\FFT{{\bfF \CM \FT}}
\def\GT{{\bfG^T}}
\def\GTG{{\GT \CDinv \bfG}}
\def\GGT{{\bfG \CM \GT}}
\def\wdhtbff{{\widehat {\bf f}}}
\def\wdhtbfx{{\widehat  \bfx }}
\def\wdhtbfX{{\widehat  \bfx }}
\def\wdhtf{{\widehat f}}
\def\wdhtg{{\widehat g}}
\def\wdhtx{{\widehat x}}
\def\wdhtbfp{{\widehat {\bf p}}}
\def\wdhtbfs{{\widehat {\bf s}}}
\def\wdhtbfS{{\widehat {\bf S}}}
\def\wdhtp{{\widehat p}}
\def\wdhtS{{\widehat S}}
\def\wdhtbfkappa{{\widehat {\bfkappa}}}
\def\wdhtkappa{{\widehat {\kappa}}}
\def\strain{{\varepsilon}}
\def\stress{{\sigma}}
\def\AND{{\sc and}}
\def\OR{{\sc or}}
\def\NOT{{\sc not}}

\def\partialderiv#1#2{{{\partial #1} \over{\partial #2}}}
\def\partialderivsquared#1#2{{{\partial^2 #1} \over{\partial #2^2}}}
\def\div{{\rm div}}
\def\grad{{\bf grad}}
\def\gradient{\widehat{\mbox{\boldmath $\gamma$}}}
\def\jacobian#1#2{\left[\partialderiv{(#1)}{(#2)}\right]}
\def\dualprod#1#2{\langle \ #1 \ , \ #2 \ \rangle}
\def\scalprod#1#2{( \ #1 \ , \ #2 \ )}
\def\scalarprod#1#2{( \ #1 \ , \ #2 \ )}

\def\implies{{\Rightarrow}}
\def\iff{{\Leftrightarrow}}
\def\IFF{{\Longleftrightarrow}}
\def\chvar{{\rightleftharpoons}}
\def\EndOfExample{{\sc[end of example.]}}

\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calI{{\cal I}}
\def\calM{{\cal M}}
\def\calP{{\cal P}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calX{{\cal X}}

\def\ND{{\rm ND}}
\def\NM{{\rm NM}}

\def\({\left(}
\def\){\right)}

%\def\begeq{\begin{equation}}
%\def\endeq{\end{equation}}
\def\begeqarray{\begin{eqnarray}}
\def\endeqarray{\end{eqnarray}}


%%% end AT defs %%%%%

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % The Newtheorem Context
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

\newtheorem{Example}{Example}%[section]
\newtheorem{Postulate}{Postulate}%[section]
\newtheorem{Lemma}{Lemma}%[section]
\newtheorem{Theorem}{Theorem}%[section]
\newtheorem{Proposition}{Proposition}%[section]
\newtheorem{Corollary}{Corollary}%[section]
\newtheorem{Property}{Property}%[section]
\newtheorem{Conjecture}{Conjecture}%[section]
\newtheorem{Proof}{Proof}%[section]
\newtheorem{Demonstration}{Demonstration}%[section]
\newtheorem{Definition}{Definition}%[section]
\newtheorem{Comment}{Comment}%[section]
\newtheorem{Algorithm}{Algorithm}%[section]
\newtheorem{Procedure}{Procedure}%[section]

\setcounter{secnumdepth}{1}
\setcounter{tocdepth}{2}

